Full-stack evaluation of Machine Learning inference workloads for RISC-V systems

Architectural simulators hold a vital role in RISC-V research, providing a crucial platform for workload evaluation without the need for costly physical prototypes. They serve as a dynamic environment for exploring innovative architectural concepts, enabling swift iteration and thorough analysis of performance metrics. As deep learning algorithms become increasingly pervasive, it is essential to benchmark new architectures with machine learning workloads. The diverse computational kernels used in deep learning algorithms highlight the necessity for a comprehensive compilation toolchain to map to target hardware platforms. This study evaluates the performance of a wide array of machine learning workloads on RISC-V architectures using gem5, an open-source architectural simulator. Leveraging an open-source compilation toolchain based on Multi-Level Intermediate Representation (MLIR), the research presents benchmarking results specifically focused on deep learning inference workloads. Additionally, the study sheds light on current limitations of gem5 when simulating RISC-V architectures, offering insights for future development and refinement.

==> conc.tex <==
\section{Conclusion}\label{sec:conc}

Our analysis of the experimental results seem to confirm that our goal of achieving fidelity is in sight. Given limited time simulations on both SST-gem5 and on VCU128 FPGA produced useful results across a number of ML inference benchmarks. Provided that the methodology flow was debugged using just 1 simple test (performing addition), the next one being MNIST and then MOBILENETv1, it is a good sign that once the initial IREE on Zephyr compatibility issues were solved all other benchmarks could run automatically.

Adaptation of Zephyr Kconfig system to support the configuration of our gem5 model as well as our FPGA softcore turned out to be straightforward. From the same codebase, we are able to build images that can be deployed to both platforms. Once the BSP was ready, compilation of the iree-run-module app as well as of the IREE runtime library files proceeded automatically, since POSIX compliance of Zephyr guarantees portability.

\subsection{Future work}

Our current efforts are focused on completing the analysis and following up on the modeling issues described above. We plan to gather empirical evidence that our SST-gem5 approach scales with the number of simulated RISC-V cores. Also, we are tracking the development of new RISC-V custom instructions' support in gem5 and softcores, mainly focusing on RVV and matrix operations extensions. These will greatly improve both simulated and simulation times and provide a more reastic platform for ML applications.

==> experiment.tex <==
\section{Experiment}

\label{sec:exp}
Following our methodology from Figure \ref{fig:overall_flow} we have reused a set of common benchmarks available from the IREE sources, which include 18 ML models, ranging from lightweight MNIST at the one end of the spectrum to GPT2 with 1.5 billion parameters. The experiments were carried out both in SST-gem5 simulation framework and RISC-V softcore emulated on FPGA. The architectural specifications of the target systems have been captured in Table \ref{tab:arch-specs}. Three CPU models in gem5 have been targeted, namely, Atomic, Minor (in-order CPU) and O3 CPU each running at 2 GHz frequency. The Memory hierarchy includes the classical caches of gem5 and simpleMem model of SST.   

\begin{table}[ht]
\centering
\caption{List of benchmarks used for evaluation.}
\label{tab:benchmarks}
\resizebox{\columnwidth}{!}{
\begin{tabular}{cccccc}\bottomrule
\textbf{Task} & \textbf{Benchmark} & \textbf{Input Dimension(s)} & \textbf{Output Dimension} & \textbf{Size(MB)} & \\\hline
Classification & Simple embedding & $1\times2\times3\times4\times$f32 (float\_32) & $1\times4$ &-  & \\ \hline
DigitRecognition  & MNIST & $1\times28\times28\times1\times$f32 (float\_32) & $1\times10$ &11.6  & \\ \hline
PoseEstimation  & Posenet & $1\times192\times192\times3\times$i8 (int\_8) & $1\times1\times\times17\times3$ &4.7  & \\ \hline
Vision  & Efficientnet lite0 & $1\times224\times224\times3\times$ui8 (unsigned\_int\_8) & $1\times1000$ &5  & \\ \hline
Classification & Mobilenet v2 & $1\times224\times224\times3\times$f32 (float\_32) & $1\times1001$ & 13.3 & \\ \hline
CreativeAI  & Magenta & $1\times256\times256\times3\times$f32 (float\_32) & $1\times1\times1\times100$ &2.5  & \\ \hline
Classification & Mobilenet V1 & $1\times224\times224\times3\times$f32 (float\_32) & $1\times1001$ &16.12  & \\ \hline
EfficientClassification  & Squeezenet & $1\times224\times224\times3\times$f32 (float\_32) & $1\times1001$ & 4.8 & \\ \hline
Segmentation  & Deeplab V3 v2 & $1\times257\times257\times3\times$f32 (float\_32) & $1\times257\times257\times21$ &2.7  & \\ \hline
ObjectDetection  & SSD Mobilebet V1 & $1\times320\times320\times3\times$ui8 (unsigned\_int\_8) & $1\times20\times20\times12$ & 6.65  & \\ \hline
Stylization  & Imagestylization & $1\times256\times256\times3\times$f32 (float\_32) & $1\times1\times1\times100$ &  9& \\ \hline
\toprule
 & & & & &\\
 & & & & &\\
\end{tabular}}
\end{table}

Running this benchmarks required a functional IREE runtime which we have ported into the Zephyr framework, and extended with 64-bit support as well as with a number of modifications required for leaner POSIX dependency (original version used some Linux-specific APIs), and for robustness in situations where multiple runs of the same app for different ML models is required.

\begin{table}
\centering
\caption{Simulated/Emulated architecture platforms}
\label{tab:arch-specs}
\begin{tblr}{
  width = \linewidth,
colspec = {Q[175]Q[192]Q[192]Q[192]Q[185]},
  cells = {c},
  cell{1}{2} = {c=3}{0.576\linewidth},
  vlines,
  vline{2} = {-}{solid,black},
  vline{2} = {2}{-}{solid,black},
  vline{3-4} = {2-7}{dashed},
  hline{1-2,8} = {-}{},
}
\textbf{Parameter}                         & \textbf{SST-gem5} &                  &                  & \textbf{FPGA}  \\
\textbf{Core Type}                         & Atomic-CPU        & Minor-CPU        & O3-CPU          & In-order       \\
\textbf{Core Frequency}                    & 2 GHz             & 2 GHz            & 2 GHz            & 100 MHz        \\
% \textbf{Core Specifications}               & RV64XX            & RV64XX           & RV64XX           & RV65GC         \\
\textbf{L1 Cache}                          & 64KB, 4-way       & 64KB, 4-way      & 64KB, 4-way      & 16KB, 64-way   \\
%textbf{L2 Cache}                          & 8MB, 4-way        & 8MB, 4-way       & 8MB, 4-way       & None           \\
\textbf{RAM Type}                          & simpleMem (SST)  & simpleMem (SST) & simpleMem (SST) & DDR4           \\
{\textbf{RAM Size}\\\textbf{Freq.}} & 3GB @ 1 GHz        & 3GB @ 1 GHz       & 3GB @ 1 GHz       & 4.5GB @ 100MHz 
\end{tblr}
\end{table}

For this paper we performed a limited set of experiments:

\begin{enumerate}

\item The normalised \emph{Execution Time} of the workloads in SST-gem5 has been depicted in Figure \ref{fig:exectime} with the MinorCPU model being the most performant. This can be attributed to the control overhead associated with O3 model (scheduling and Re-ordering) whereas the workloads in our setup are expected to be spending a significant time in pure compute as we only measure kernel execution time for inference.

\begin{figure}
\caption{Normalized execution time for each workload on Gem5}
\label{fig:exectime}
\includegraphics[height=.6\columnwidth,width=\columnwidth]{figs/Exec_gem5.pdf}
\end{figure}

\item A preliminary comparison showing impact of O3 vs. in-order model is shown in Figure \ref{fig:comparison}.

%removed IPC as all were close to 0.99
\begin{figure}[hbt]
\caption{Comparison on gem5 using O3 vs. in-order core}
    \includegraphics[height=.6\columnwidth,width=\columnwidth]{figs/o3_vs_minor.pdf}
\label{fig:comparison}
\end{figure}

% \begin{figure}
% \caption{Normalized Runtime overhead each workload on Gem5}
% \end{figure}
\item Because running the models on the FPGA that expose much micro-archtitectural state is limited to a simple cycle counter, we can report here only the absolute execution cycle times in Figure \ref{fig:fpga}.

\begin{figure}
\caption{Workload execution time for Rocket core in VCU128}
\includegraphics[height=.6\columnwidth,width=\columnwidth]{figs/Cycles-FPGA.pdf}
\label{fig:fpga}
\end{figure}

\item Finally, we report the Misses Per Kilo Instructions (MPKI) for the workloads running on various gem5 CPU models. General trend seems to be as expected, however, the impact of running the (in-order) MinorCPU shows much larger deviation from AtomicCPU, which could indicate an issue in modeling.

\begin{figure}
\caption{MPKI for each workload on gem5}
\includegraphics[height=.6\columnwidth,width=\columnwidth]{figs/MPKI.pdf}
\end{figure}

\end{enumerate}

% \begin{figure}
% \caption{Simulation time speedup on FPGA compared to Gem5}
% \includegraphics[width=\columnwidth]{figs/fpga_speedup.pdf}
% \end{figure}
% % Not sure about this graph, please check. -Anmol

% \begin{figure}
% \caption{Memory footprint of the workload running on Gem5}
% \end{figure}

% \begin{figure}
% \caption{Speedup in execution time on enabling vector extensions}
% \end{figure}


\begin{figure}
\end{figure}


==> methodology.tex <==
\section{Methodology}\label{sec:method}
\noindent While custom instructions and hardware accelerators offer performance improvements for specific machine learning tasks, we 
choose the RISC-V~\texttt{RV64GC+f} architecture as a baseline for benchmarking purposes. Firstly, employing the baseline architecture ensures a standardized and repeatable benchmark environment. This allows for fair comparisons between different ML models and algorithms, as the underlying hardware platform remains consistent. Deviation from this baseline introduces the risk of performance gains being attributed to hardware-specific optimizations, rather than inherent model or algorithm improvements. 
Secondly, utilizing a readily available and open-source architecture like RISC-V~\texttt{RV64GC+f} significantly reduces development time and complexity. Researchers and developers can readily leverage existing tools and resources for benchmarking purposes, eliminating the need for specialized hardware or custom software development. Furthermore, the baseline RISC-V architecture offers greater flexibility and extensibility for benchmarking diverse ML workloads. Unlike custom architectures, which may be optimized for specific tasks, the RISC-V instruction set remains general-purpose, allowing for the evaluation of a wider range of models and algorithms. This enables wider adoption and evaluation of various ML tasks.
%\todoi{How to justify lack of V?}

\begin{figure}[t]
    \centering
    \includegraphics*[width=\columnwidth]{figs/overall.png}
    \caption{Methodology for evaluation of deep learning models on RISC-V hardware platforms}
    \label{fig:overall_flow}
\end{figure}

The overall flow where we stipulate the necessity of leveraging standard tools and frameworks, portability and reuse is shown in Figure \ref{fig:overall_flow} and further detailed below.

\subsection{A case for SST-gem5 integration}
For the experimental part of this work, we have employed software tools to define and simulate our hardware platform, comparing the results and calibrating design parameters against a real FPGA RISC-V softcore. Specifically, a combination of two tools has been used: The gem5 simulator \cite{DBLP:journals/corr/abs-2007-03152} and the Structural Simulation Toolkit (SST) \cite{10.1145/1964218.1964225}.

The gem5 simulator is an open-source high-level system simulator, with contributions from numerous individuals, universities, and companies too. We have decided to adopt this tool for our CPU core implementation, due to its flexibility and complete compatibility with the RISC-V ISA.
Because discrete-event simulation of modern cores requires detailed modeling of all stages of the pipeline, such simulations are often slow. This bottleneck also prevents simulations to scale to a large number of cores. To alleviate this problem, we have utilized SST as a {\em parallel} discrete-event simulator which is capable of distributing simulated architecture across a cluster using MPI. 

\subsection{RISC-V Rocket Core}
% The first sentence may change to "glue" it to the previous para
The low throughput of architectural simulators - often few thousands Kilo Instructions Per Second (KIPS) - hinders the exploration of larger workloads with detailed models. FPGAs provide a means to accelerate the design explorations by increasing the throughput with little design overhead. We emulate the open source Rocket-chip based on RISC-V ISA (citation needed) on VCU128 Ultrascale+ FPGA. The high level view of the system is depicted in Figure \ref{fig:Rocket-Core}. The board has 4.5GB of DDR4 DRAM. The rocket chip comprises of a single 5 stage in-order core with (pipelined) single and double precision fused multiply and accumulate units synthesised on DSP48E1 slices. The Functional Units include (10 cycle latency) iterative integer multiplier, single-cycle latency ripple carry adder and integer division unit. The front-end of the core comprises of a Gshare branch predictor that uses hash of PC and Global history to index into the Pattern History Tables. It has a 32-entry Return Address Stack. Both the Rocket core and DRAM operate at a frequency of 100MHz. The Rocket tile comprises of the core has L1 instruction and data cache.
% Glue to the next para describing u-architecture
\begin{figure}
    \centering
    \includegraphics*[trim = 0 120mm 0 35mm , width=\columnwidth]{figs/Rocket-Detailed.pdf}
    \caption{Simplified architecutre of Rocket SoC in VCU128}
    \label{fig:Rocket-Core}
\end{figure}

\begin{figure}
    \centering
    \includegraphics*[trim = 0mm 50mm 50mm 0 , width=\columnwidth]{figs/rocket_util.pdf}
    \caption{Resource Utilization of Rocket SoC emulated on VCU128 Ultrascale+}
    \label{fig:Rocket-Core}
\end{figure}


\subsection{MLIR based representation of ML models}
With the widespread adoption of ML, a large number of machine learning 
frameworks have evolved over time. Some of the widely used ones include PyTorch, Tensorflow, ONNX and Caffe.  Even though most of the frameworks are available with a Python frontend, they have their own operator sets alongwith specific implementations of runtime. From the perspective of hardware developers, this leads to high development and testing overhead, since the runtime has to be ported for the specific hardware.

In order to get around this problem, we focus on using MLIR representation of the ML models~\cite{lattner2021mlir}. MLIR offers a modern open source compiler infrastructure for multi-level intermediate representations and it resides as a subproject inside LLVM~\cite{lattner2004llvm}. To enable representation of ML models in MLIR, different dialects and optimization passes have been defined. A {\em dialect} serves as
an abstraction or intermediate representation, and an
optimization pass is to enable optimization at an abstraction
level or transformation among abstraction levels. MLIR offers high level dialects such as Tensor Operator Set Architecture~(TOSA)~\cite{tosa} which can effectively capture the semantics of modern deep learning based ML models. Multiple ML frameworks currently support exporting models into MLIR based representations. eg: Tensorflow-MLIR\footnote{https://github.com/tensorflow/tensorflow/tree/master/tensorflow/compiler/mlir}, PyTorch-MLIR\footnote{https://github.com/llvm/torch-mlir}, ONNX-MLIR\footnote{https://github.com/onnx/onnx-mlir}, etc. 
%An example of MLIR based representation of Lenet5~\cite{lenet5} is shown in Fig.~\ref{fig:code_layout}.

\begin{figure*}
    \centering
        \begin{minipage}{\textwidth}
    {\footnotesize
        \begin{lstlisting}
module attributes {torch.debug_module_name = "ModelLenet5"} {
      func.func @forward(%arg0: tensor<1x1x28x28xf32>) -> tensor<1x10xf32> {
      %0 = "tosa.const"() <{value = dense<"0x98B78CBCF0EA633C8A4442BDD057B..."
      ...
      %43 = "tosa.matmul"(%41, %42) : (tensor<1x1x84xf32>, tensor<1x84x10xf32>) -> tensor<1x1x10xf32>
      %44 = "tosa.reshape"(%43) <{new_shape = array<i64: 1, 10>}> : (tensor<1x1x10xf32>) -> tensor<1x10xf32>
      %45 = "tosa.add"(%44, %12) : (tensor<1x10xf32>, tensor<1x10xf32>) -> tensor<1x10xf32>
      %46 = "tosa.clamp"(%45) <{max_fp = 3.40282347E+38 : f32, max_int = 2147483647 : i64, min_fp = 0.000000e+00 : f32, min_int = 0 : i64}> : (tensor<1x10xf32>) -> tensor<1x10xf32>
      return %46 : tensor<1x10xf32>
      }
}
        \end{lstlisting}
        }
        \end{minipage}
    \caption{A snippet of the Lenet5 model~(\texttt{model.mlir}) in MLIR format, represented in TOSA dialect. MLIR uses three-address static single assignment (SSA)-based Intermediate Representation, similar to LLVM. We can see that operations like {\em matmul} are directly represented, from the TOSA dialect}
    \label{fig:code_layout}
\end{figure*}



\subsection{Compilation of MLIR models}
In this work, we use the open-source IREE (Integration, Representation, and Execution Environment) framework for compilation. IREE has been developed by Google, for compiling, optimizing, and executing machine learning models  represented in MLIR across a variety of hardware targets~\cite{liu2022tinyiree}. IREE offers a runtime that relies on a lightweight virtual machine to address the challenge of deploying machine learning models across diverse hardware environments efficiently. It supports multiple hardware targets out-of-the-box,  such as CPUs and GPUs. IREE uses MLIR based infrastructure for optimization of the ML models for efficient code generation. IREE offers the flexibility to abstract away hardware-specific optimizations and allows streamlined deployment of machine learning models. The compiled model is stored in a flatbuffer format, which is parsed by the IREE runtime during inference. A representative compilation command is presented in Fig.~\ref{fig:iree_compile}. The flatbuffer embeds instruction for orchestration of the runtime as well as native instructions for the target hardware for each computation kernel.

\begin{figure}[ht]
    \centering
    {\footnotesize
    \begin{lstlisting}[language=bash]
iree-compile
--iree-hal-target-backends=llvm-cpu \
--iree-llvm-target-triple=riscv64 \
--iree-llvm-target-cpu-features=+m,+a,+f,+d,+c\
--iree-input-type=tosa \
--print-pipeline-passes \
--iree-hal-dump-executable-sources-to=/tmp/lenet5 \
model.mlir -o model.vmfb
    \end{lstlisting}
}

    \caption{The \texttt{iree-compile} tool is used to compile the MLIR models to a flat-buffer %\footnote{https://flatbuffers.dev/} 
format}
    \label{fig:iree_compile}
\end{figure}

\subsection{A case for POSIX: Zephyr}

Similar to portability concerns leading to the use of a virtual machine for the orchestration layer of IREE-compiled models, its runtime requires a standardized base functionality to function appropriately. While is is certainly possible to re-implement IREE runtime library on various new platforms such as baremetal or FreeRTOS, doing so is quite involved as many required features already supported by e.g., Linux (by far the most popular platform for ML) would need to ported to run on a completely different set of APIs. And also verfied, of course. 

While running Linux on gem5 and FPGAs is definitely possible, however, its hardly very efficient. The whole design and common algorithms are optimized for fast out-of-order (O3) cores, while even in FPGAs, frequencies higher than 100Mhz are rarely attainable. This makes tuning Linux for this - almost embedded usage - not a trivial task. For example, shared libraries introduce various inefficiencies while the separation between kernel- and user-space causes many unrelated issues to surface. Besides we're hardly interested in running generic Linux applications securely in a multi-user environment, rather only a bare minimum required by the IREE runtime.

An alternative strategy is to retain a common API - POSIX - and leverage an embeddable libray OS (a nano-kernel) that supports it. For us, Zephyr is the perfect choice: (1) it implements a large subset of POSIX, (2) highly customizable to the most meagre platforms, (3) supporting various C libraries such a picolibc \& newlib and (4) offers a integrated build system for library and application development.
The architecture of Zephyr is depicted in Figure \ref{fig:Zephyr-POSIX}.

\begin{figure}
    \centering
    \includegraphics*[width=1\columnwidth]{figs/posix.png}
    \caption{Zephyr POSIX architecture}
    \label{fig:Zephyr-POSIX}
\end{figure}


Because of the current lack of support for storage subsystem (and the difficulties in setting up a shared model space) in gem5, we opted to make use of a ramdisk-based filesystem, embedded into the ELF image generated by Zephyr. We follow same approach that IREE mandates: the usage of iree-run-module tool that is capable of launching any ML model by running it either natively (on Linux) or in gem5/FPGA (on Zephyr).

\begin{figure}[ht]
    \centering
    {\footnotesize
    \begin{lstlisting}[language=bash]
iree-run-module
--device=local-task
--module=/RAM:/mnist.vfb
--function=predict
--input=1x28x28x1xf32=@/RAM:/mnist.bin
    \end{lstlisting}
}
    \caption{The \texttt{iree-run-module} tool invocation for a model}
    \label{fig:iree_run}
\end{figure}

